Near-Optimal Tensor PCA via Normalized Stochastic Gradient Ascent with Overparameterization

We study the Order-$k$ ($k \geq 4$) spiked tensor model for the tensor principal component analysis (PCA) problem: given $N$ i.i.d. observations of a $k$-th order tensor generated from the model $\mathbf{T} = \lambda \cdot v_*^{\otimes k} + \mathbf{E}$, where $\lambda > 0$ is the signal-to-noise ratio (SNR), $v_*$ is a unit vector, and $\mathbf{E}$ is a random noise tensor, the goal is to recover the planted vector $v_*$. We propose a normalized stochastic gradient ascent (NSGA) method with overparameterization for solving the tensor PCA problem. Without any global (or spectral) initialization step, the proposed algorithm successfully recovers the signal $v_*$ when $N\lambda^2 \geq \widetilde{\Omega}(d^{\lceil k/2 \rceil})$, thereby breaking the previous conjecture that (stochastic) gradient methods require at least $\Omega(d^{k-1})$ samples for recovery. For even $k$, the $\widetilde{\Omega}(d^{k/2})$ threshold coincides with the optimal threshold under computational constraints, attained by sum-of-squares relaxations and related algorithms. Theoretical analysis demonstrates that the overparameterized stochastic gradient method not only establishes a significant initial optimization advantage during the early learning phase but also achieves strong generalization guarantees. This work provides the first evidence that overparameterization improves statistical performance relative to exact parameterization that is solved via standard continuous optimization.

==> Main_Latex/Algorithm.tex <==
\begin{algorithm}[t]
	\caption{Stochastic Gradient Ascent (SGA)}
	\label{SGA}
	\hspace*{0.02in}{\bf Input: }Initial weight $W^{(0)}=I_d\in\bbR^{d\times d}$, initial step-size $\eta_0$, total sample size $T$, decaying phase length $T_1=\left\lfloor T/\log(T)\right\rfloor$.
	\\
	\hspace*{0.02in}{\bf Output: }$v_{\mathrm{Alg}}\in\bbR^d$.
	\begin{algorithmic}[1] 
		\WHILE{$t\leq T$}
		\IF{$t>0$ and $t$ mod $T_1=0$}
		\STATE $\eta_0\leftarrow\eta_0/2$.
		\ENDIF
		\STATE Sample a fresh data $\upT^{(t+1)}$.
		\STATE $W^{(t+1)}\leftarrow W^{(t)}+\eta_0\nabla_{W}\hatcR(W^{(t)})$.
		\ENDWHILE
		\STATE Computing $v_{\mathrm{Alg}}$ to approximate the top  eigenvector of matrix $\frac{1}{2}\left(W^{(T)}+(W^{(T)})^{\top}\right)$ via the power method.
	\end{algorithmic}
\end{algorithm}
Stochastic Gradient Descent (SGD) and its variants are the algorithms of choice for solving many complex minimization problems in machine learning and data science. Analogously, for maximization problems, SGA can optimize reward functions. To recover the signal vector $v_*$, we leverage the structure of Problem \ref{PCA-def} to design a specialized reward function and parameterization, subsequently solving it via SGA. For even $k$, we parameterize the solution as a matrix $W\in\bbR^{d\times d}$ and define the reward function as:
\begin{align}\label{PCA-aux-reward}
	\calR_{\mathrm{even}}(W):=\bbE\left[\hatcR_{\mathrm{even}}(W):=\frac{1}{\left\|W\right\|_{\tF}^{\frac{k}{2}-2}}\llangle W^{\otimes\frac{k}{2}},\upT\rrangle\right],
%	=\frac{1}{\left\|W\right\|_{\tF}^{\frac{k}{2}-2}}\bbE\left[\llangle W^{\otimes\frac{k}{2}},\lambda\cdot v_*^{\otimes k}+\upE\rrangle\right],
\end{align}
where $W\in\bbR^{d\times d}$ is an  overparameterized parameter matrix. 

Existing studies demonstrate that overparameterized stochastic gradient methods efficiently approximate optimal solutions, as seen in quadratically parameterized models \cite{woodworth2020kernel,haochen2021shape,ding2025scaling} and matrix factorization models \cite{tu2016low,li2018algorithmic,xiong2023how}. Inspired by these approaches, we use $W\in\bbR^{d\times d}$ to approximate $v_*v_*^{\top}$. Since $v_*v_*^{\top}$ has a unit Frobenius norm, we introduce the normalization factor $1/\left\|W\right\|_{\tF}^{\frac{k}{2}-2}$ in the reward function to constrain growth of $\left\|W\right\|_{\tF}$ during optimization. We optimize $W$ via SGA using $\hatcR=\hatcR_{\mathrm{even}}$, as detailed in Algorithm \ref{SGA}.

Our step-size strategy employs a tail geometric decay strategy \cite{wu2022last}: it remains constant for the first $T_1=\lfloor T/\log(T)\rfloor$ iterations, then halves every $T_1$ steps thereafter. Combining warm-up initialization with learning rate decay is prevalent in deep learning optimization \cite{goyal2017accurate}. Geometric decay strategy are empirically superior to polynomial decay within the decay stage, as they effectively balance aggressive early learning with stable late-stage refinement \cite{ge2019step}. Motivated by these advantages, our step-size strategy integrates an initial constant phase with subsequent geometric decay. 

%This hybrid approach leverages the computational efficiency of geometric decay while retaining the stability benefits of warm-up, achieving synergistic effects unattainable with polynomial decay \cite{bubeck2015convex}.可以放到理论分析中进行讨论

When $k$ is odd, a preprocessing step is applied to the tensor $\upT$ obtained at each sampling iteration. Given a preprocessing unit vector $u\in\bbR^d$, we construct a new preprocessed tensor $\upT(u)\in\otimes^{k-1}\bbR^d$ according to the definition in Section \ref{prelimin} (\emph{tensor manipulation}). Consider the associated reward (loss) function:
\begin{align}
	\calR_{\mathrm{odd}}(W):=\bbE\left[\hatcR_{\mathrm{odd}}(W):=\frac{1}{\left\|W\right\|_{\tF}^{\frac{k-1}{2}-2}}\llangle W^{\otimes\frac{k-1}{2}},\upT(u)\rrangle\right].
\end{align}
One can notice that the tensor $\upT(u)$ resulting from this preprocessing is an even-order tensor exhibiting a structure analogous to the observed tensor in Problem \ref{PCA-def}--specifically, it comprises a principal component and a random noise matrix. However, the optimization requires concurrent execution of both maximizing $\calR_{\mathrm{odd}}$ and $-\calR_{\mathrm{odd}}$ by SGA due to sign ambiguity in the SNR $\lambda\langle v_*,u\rangle$ of the principal component for $\upT(u)$. Pseudocode for optimizing the weight matrix $W$ when $k$ is odd is provided in Algorithm \ref{k-odd}. 
%we first note that $\upT$ can be decomposed into $d$ slices $\left\{\upT_i\right\}_{i=1}^d$, where each slice  $\upT_i\in\otimes^{k-1}\bbR^d$ is a sub-tensor satisfying
%\begin{align}
%	\upT_i=v_*(i)\cdot v_*^{\otimes(k-1)}+\upE_i,\notag
%\end{align}
%The collection of random tensor slices $\left\{\upE_i\right\}_{i=1}^d$ can be concatenated to form the tensor $\upE$. Subsequently, leveraging the vector $u$, 
%we construct a new preprocessed tensor $\upT(u)\in\otimes^{k-1}\bbR^d$ defined as follows:
%\begin{align}
%	\upT(u)=\sum_{i=1}^d u(i)\cdot\upT_i.\notag
%\end{align}
\begin{algorithm}[t]
	\caption{Bi-Threaded SGA}
	\label{k-odd}
	\hspace*{0.02in}{\bf Input: }Initial weight $W^{(0)}=I_d\in\bbR^{d\times d}$, initial step-size $\eta_0$, total sample size $T$, decaying phase length $T_1=\left\lfloor T/\log(T)\right\rfloor$,  preprocessing unit vector $u\in\bbR^d$.
	\\
	\hspace*{0.02in}{\bf Output: }$v_{\mathrm{Alg}}\in\bbR^d$.
	\begin{algorithmic}[1]
		\STATE Execute two parallel instances of the SGA (Algorithm \ref{SGA}), where the first instance employs the reward function $\hatcR=\hatcR_{\mathrm{odd}}$, and the second instance employs the reward function $\hatcR=-\hatcR_{\mathrm{odd}}$.
		\STATE  The first instance yields an output value denoted as $v_{\mathrm{Alg}}^{(1)}$, while the second instance yields an output value denoted as $v_{\mathrm{Alg}}^{(2)}$. Randomly pick up $v_{\mathrm{Alg}}^{(l)}$ from $l\in\{1,2\}$ following the probability $\bbP[l]=0.5$ as $v_{\mathrm{Alg}}$.
	\end{algorithmic}
\end{algorithm}

Algorithm \ref{SGA} and Algorithm \ref{k-odd} share a common core: both implement SGA with a geometrically decaying step-size. This finite-horizon online algorithm simultaneously achieves the timeliness inherent to online methods and matches the optimal sample complexity of state-of-the-art solvers for Problem \ref{PCA-def} (see Section \ref{tensor} for proof).

==> Main_Latex/preliminary.tex <==
\subsection{Notations}
\noindent\textbf{Linear algebra. }We denote real vectors by lowercase letters (e.g., $u,v$) and real matrices by uppercase letters (e.g., $Q,W,X$). A vector in $\bbR^d$ is written as $x=\left(x(1),\cdots,x(d)\right)$, and a matrix in $\bbR^{d\times d}$ as $W=\left(W(i,j)\right)_{d\times d}$. The orthogonal complement of a vector $v$ is defined by $v_{\perp}$. For $n\in\bbN_+$, $[n]$ represents the set $\{1,\cdots, n\}$. For functions $f,g:\bbR\rightarrow\bbR$, we write $f\lesssim g$ if $f=\calO(g)$, $f\gtrsim g$ if $f=\Omega(g)$, and $f\asymp g$ if $g\lesssim f\lesssim g$.
\\
\\
\noindent\textbf{Inner products and norms. } The standard entrywise inner product is denoted $\langle\cdot,\cdot\rangle$. For vectors $u,v\in\bbR^d$, $\langle u,v\rangle=\sum_{i=1}^{d}u_iv_i$. For matrices $Q,W\in\bbR^{d\times d}$, $\llangle Q,W\rrangle=\tr\left(Q^{\top}W\right)$. The $\l_2$-norm of $v\in\bbR^d$ is given by $\|v\|$. The matrix norm used throughout the paper will be the Frobenius norm, denoted by $\left\|W\right\|_{\tF}$ for matrix $W\in\bbR^{d\times d}$. Let $\calW$ be the parameter space with definition: $\calW=\left\{W\in\bbR^{d\times d}:\left\|W\right\|_{\tF}=1\right\}$. 
\\
\\
\noindent\textbf{Tensor manipulation. } Tensors of order-$k\geq 4$ are denoted by boldface uppercase letters (e.g., $\upT,\upE\in\otimes^k\bbR^d$). We denote by $\upT(\cdot):\bbR^d\rightarrow\otimes^{k-1}\bbR^d$ the multilinear function such that $\upT(x)=\left(\sum_{i=1}^dx(i_1)T(i_1,i_2,\cdots,i_k)\right)$, applying $x$ to the first modes of the tensor $\upT$. 

Tensors can be flattened into vectors via the operator $\expan:\otimes^k\bbR^d\rightarrow\bbR^{d^k}$, which reinterprets tensor indices into a lexicographic ordering and has the following form $\expan(\upT)((i_1-1)d^{k-1}+(i_2-1)d^{k-2}+\cdots+(i_{k-1}-1)d+i_k):=\upT(i_1,\cdots,i_k)$ for any $i_1,\cdots,i_k\in[1:d]$ under given tensor $\upT\in\otimes^k\bbR^d$. The inner product for tensors is defined as $\langle\upT_1,\upT_2\rangle:=\llangle\expan(\upT_1),\expan(\upT_2)\rrangle$. The $k$-fold outer product of vector $v\in\bbR^d$ is $v^{\otimes k}$.

\subsection{Noise Tensor Assumptions}
We make the following assumptions of random noise tensor $\upE$ in Problem \ref{PCA-def}.
\begin{assumption}\label{ass-2} 
    For any unit vector $u\in\bbR^{d^k}$, let $X=\langle u, \expan(\upE)\rangle$. Then there exists $\sigma>0$ such that
    \begin{align}
		\bbE\left[\exp\left\{\lambda X\right\}\right]&\leq\exp\left\{\lambda^2\sigma^2\right\},\quad \forall \lambda\in\bbR.\notag
%		\label{ass-sub-gaussian}
%		\\
%		\bbE\left[X^2\right]&=\mathsf{c}_0\sigma^2.\label{ass-moment}
    \end{align}
\end{assumption}
Assumption \ref{ass-2} implies that the vectorization $\expan(\upE)$ of the zero-mean random noise tensor $\upE$ possesses a \textit{rotationally invariant sub-Gaussian property}. Specifically, for any orthogonal matrix $Q \in \bbR^{d^k\times d^k}$, each coordinate of $Q \expan(\upE)$ is sub-Gaussian with parameter $\sigma$ (Definition \ref{sub-Gaussian}). While standard tensor PCA literature \cite{hopkins2015tensor,hopkins2016fast,arous2020algorithmic,dudeja2024stat} assumes $\upE$ has i.i.d. $\calN(0,\sigma^2)$ entries (which constitutes a special case satisfying Assumption \ref{ass-2}), our framework accommodates broader noise models. The assumption holds in particular when $\expan(\upE)$ satisfies either of the following sufficient conditions:
(1) Its coordinates are mutually independent sub-Gaussian random variables with parameter $\sigma$;
(2) The uniform bound $\left\|\expan(\upE)\right\|\leq\sigma$ holds. Furthermore, under this assumption, we derive the following moment bounds for $\expan(\upE)$.
\begin{corollary}\label{corollary-estimation-second-moment}
    Suppose Assumption \ref{ass-2} holds. For any unit vector $u\in\bbR^{d^k}$, the following second-order moment condition holds for $\llangle u,\expan(\upE)\rrangle$
    \begin{align}
    \bbE\left[\llangle u,\expan(\upE)\expan(\upE)^{\top}u\rrangle\right]\leq4\sigma^2.\notag
    \end{align}
\end{corollary}
We introduce an additional assumption on the second-order moment of $\upE$ (Assumption \ref{assumption-estimation-second-moment}), which also holds in the i.i.d. gaussian entries setting \cite{hopkins2015tensor,hopkins2016fast,arous2020algorithmic,dudeja2024stat}. However, this assumption does not compromise the convergence guarantees of Algorithm \ref{SGA} and Algorithm $\ref{k-odd}$. In Section \ref{tensor}, we further establish the convergence rates for both algorithms even in the absence of Assumption \ref{assumption-estimation-second-moment}.
\begin{assumption}\label{assumption-estimation-second-moment}
	For any unit vector $u\in\bbR^{d^k}$, there exists a constant $\mathsf{c}_0$ such that
	\begin{align}
		\bbE\left[\llangle u,\expan(\upE)\expan(\upE)^{\top}u\rrangle\right]=\mathsf{c}_0\sigma^2.\notag
	\end{align}
\end{assumption}

==> Main_Latex/tensor_PCA_APP.tex <==
%\subsection{High-Probability Results Guarantee}\label{high-probability}
%In this section, we also begin with introducing the guarantee of our constant-probability results. We formally define a series of events for each iteration of SGD. We demonstrate that these events occur with high probability throughout the whole $T$ iterations, which indicates that the control sequence $\{\tisW^{(t)}\}_{t=0}^T$ we define is aligned with the original sequence $\{W _t\}_{t=0}^T$ with high probability. This fact is the basis of our constant-probability results.
%
%Let $R(\delta,\tau_1):=\calO\left(\log\left((kT^2d^2)/\min\{\delta,\tau_1\}\right)\right)$ for failure probability $\delta\in(0,1)$ and deviation bound $\tau_1\in(0,1)$. Define the matrix value functions $\widehat{ S}_t:\bbR^{d\times d}\rightarrow\bbR^{d\times d}$ and $\breve{ S}_t:\bbR^{d\times d}\rightarrow\bbR^{d\times d}$ with following forms for any $t\in[1:T]$:
%\begin{equation}
%	\left\{
%	\begin{aligned}
%		&\llangle\widehat{ S}_t( V_1), V_2\rrangle=\sum_{i=1}^{k/2}\llangle\widehat{ S}_t^i( V_1), V_2\rrangle,
%		\\
%		&\llangle\breve{ S}_t( V_1), V_2\rrangle=\llangle \upS_t, V_1^{\otimes k/2}\rrangle\llangle V_1, V_2\rrangle,
%	\end{aligned}
%	\right. \, \, \, \, \, \, \quad \forall\,   V_1, V_2\in\bbR^{d\times d},
%\end{equation}
%where $\langle\widehat{ S}_t^i( V_1), V_2\rangle$ is defined as follows:
%$$
%\llangle\widehat{S}_t^i( V_1), V_2\rrangle=\llangle \upS_t, V_1^{\otimes(i-1)}\otimes V_2\otimes V_1^{\otimes(k/2-i)}\rrangle,
%$$
%for any $i\in[1:k/2]$. In order to simply rule out some low-probabilistic unbounded cases, we define the following events at each iteration $t$. Given matrix $ V_1\in\bbR^{d\times d}$, index $i\in[1:k/2]$ and coordinate $(i',j')\in[1:d]\times[1:d]$, let
%\begin{equation}
%	\left\{
%	\begin{aligned}
%		\calE_{1,i}^t( V_1)(i',j'):=&\left\{\left.\left|\widehat{ S}_t^i( V_1)(i',j')\right|\leq c_{1,i'j'}^i( V_1)\right|\calF_{t-1}\right\},
%		\\
%		\calE_{2}^t( V_1)(i',j'):=&\left\{\left.\left|\breve{ S}_t( V_1)(i',j')\right|\leq c_{2,i'j'}( V_1)\right|\calF_{t-1}\right\},
%	\end{aligned}
%	\right.
%\end{equation}
%where $\left\{c_{1,i'j'}^i( V_1)\right\}_{i',j'\in[1:d]}$ and $\left\{c_{2,i'j'}( V_1)\right\}_{i',j'\in[1:d]}$ depend on $ V_1$ and satisfy
%\begin{align}
%	\sum_{i'=1}^{d}\sum_{j'=1}^{d}\left(c_{1,i'j'}^i( V_1)\right)^2\leq\sigma^2\left\| V_1\right\|_{\tF}^{k-2}R(\delta,\tau_1),\quad\text{ and }\quad \sum_{i'=1}^{d}\sum_{j'=1}^{d}\left(c_{2,i'j'}( V_1)\right)^2\leq\sigma^2\left\| V_1\right\|_{\tF}^{k+2}R(\delta,\tau_1).\notag
%\end{align}
%Under Assumption \ref{ass-2}, for sufficiently large $T$, Lemma \ref{aux-truncation-subGaussian-covariance} implies
%\begin{equation}\label{expectation-pca-noise}
%	\begin{aligned}
%		&\left|\left.\bbE\left[\sum_{i'=1}^d\sum_{j'=1}^{d}\widehat{ S}_t^i( V_1)(i',j') V_2(i',j')\mathds{1}_{\calE_{1,i}^t( V_1)(i',j')}\right|\calF_{t-1}\right]\right|\leq\tau_1\left\| V_1\right\|_{\tF}^{k/2-1}\left\| V_2\right\|_{\tF},
%		\\
%		&\left|\left.\bbE\left[\sum_{i'=1}^d\sum_{j'=1}^{d}\breve{ S}_t( V_1)(i',j') V_2(i',j')\mathds{1}_{\calE_{2}^t( V_1)(i',j')}\right|\calF_{t-1}\right]\right|\leq\tau_1\left\| V_1\right\|_{\tF}^{k/2+1}\left\| V_2\right\|_{\tF},
%	\end{aligned}
%\end{equation}
%for any $i\in[1:k/2]$. Moreover, utilizing Proposition \ref{prop-A5}, we obtain
%\begin{equation}\label{control-prob-PCA-1}
%	\begin{aligned}
%		\min\left\{\bbP\left(\calE_{1,i}^{t}( V_1)(i',j')\right),\bbP\left(\calE_{2}^{t}( V_1)(i',j')\right)\right\}\geq 1-\calO\left(\frac{\delta}{T^2\poly(kd^2)}\right),
%	\end{aligned}
%\end{equation}
%for any $t\in[1:T]$. For simplicity, we define random matrices $\widetilde{\widehat{ S}}_t^i( V_1)$ and $\widetilde{\breve{ S}}_t( V_1)$ as follows:
%\begin{equation}\label{component-tiSt}
%	\left\{
%	\begin{aligned}
%		&\widetilde{\widehat{ S}}_t^i( V_1)(i',j'):=\widehat{ S}_t^i( V_1)(i',j')\mathds{1}_{\calE_{1,i}^t( V_1)(i',j')},
%		\\
%		&\widetilde{\breve{ S}}_t( V_1)(i',j'):=\breve{ S}_t( V_1)(i',j')\mathds{1}_{\calE_2^t( V_1)(i',j')},
%	\end{aligned}
%	\right.\, \, \, \, \, \quad \forall i',j'\in[1:d],
%\end{equation}
%for any $ V_1\in\bbR^{d\times d}$ and index $i\in[1:k/2]$. According to the update rule of $W _t$ in Eq.~\eqref{SGD-tensor-PCA} and the definition of $ S_{W _t}$ in Eq.~\eqref{define-SW_t}, we define the compound event as 
%\begin{align}
%	\calE^t:=\bigcap_{i',j'\in[1:d]}\left(\left(\bigcap_{i=1}^{k/2}\calE_{1,i}^t(W _{t-1})(i',j')\right)\bigcap\calE_2^t(W _{t-1})(i',j')\right).
%	\notag
%\end{align}
%Utilizing Eq.~\eqref{control-prob-PCA-1}, we can directly obtain the probability union bound as follows:
%\begin{align}
%	\bbP\left(\bigcap_{t=1}^T\calE^t\right)=&1-\bbP\left(\bigcup_{t=1}^T(\calE^t)^c\right)\notag
%	\\
%	\geq&1-\sum_{t=1}^T\sum_{i'=1}^{d}\sum_{j'=1}^{d}\left(\frac{k}{2}+1-\sum_{i=1}^{k/2}\bbP\left(\left(\calE_{1,i}^t(W _{t-1})(i',j')\right)^c\right)-\bbP\left(\left(\calE_2^t(W _{t-1})(i',j')\right)^c\right)\right)\notag
%	\\
%	\geq&1-\calO\left(\frac{\delta}{T}\right).\notag
%\end{align}



%For simplicity, we define the random tensor $\tisE^{(t)}:=E^{(t)}\cdot\mathds{1}_{\calA_{1}^{(t)}(\delta)\cap\calA_{2}^{(t)}(\delta)}$. The high-probability occurrence of event $\bigcap_{t=0}^{T-1}\left(\calA_{1}^{(t)}(\delta)\cap\calA_{2}^{(t)}(\delta)\right)$ provided by Lemma \ref{lemma:high-prob} guarantees our analysis of dynamics for the control sequence $\left\{\tisW^{(t)}\right\}_{t=0}^{T}$ defined in $\bbR^{d\times d}$ as
%\begin{equation}\label{SGD-tensor-PCA-control-sequence}
%	\begin{split}
%		\tisW^{(t+1)}=&\tisW^{(t)}+\frac{\eta_t\lambda k}{2}\cdot\frac{\langle v_*,\tisW^{(t)} v_*\rangle^{\frac{k}{2}-1}}{\left\|\tisW^{(t)}\right\|_{\text{F}}^{\frac{k}{2}-2}}\cdot v_* v_*^{\top}-\frac{\eta_t\lambda(k-4)}{2}\cdot\frac{\llangle v_*,\tisW^{(t)} v_*\rrangle^{\frac{k}{2}}}{\left\|\tisW^{(t)}\right\|_{\text{F}}^{\frac{k}{2}}}\cdot\tisW^{(t)}+\eta_t\tisE^{(t)},
%		\\
%		=&\tisW^{(t)}+\eta_t\nabla\widehat{\calR}(\tisW^{(t)}),
%	\end{split}
%\end{equation}
%with initialization $\tisW^{(0)}=W^{(0)}$ for any $t\in[0:T-1]$, where  matrix $\tisE^{(t)}$ obeys Eq.~\eqref{def-E} when the substitutions of $W^{(t)}$ with $\tisW^{(t)}$ and $E^{(t)}$ with $\tisE^{(t)}$ are respectively made. Similarly, the events $\calA_{1}^{(t)}(\delta)$ and $\calA_{2}^{(t)}(\delta)$ still adhere to the definitions in Lemma \ref{lemma:high-prob}, with the only modification being the substitution of $E^{(t)}$ by $\tisE^{(t)}$ and $W^{(t)}$ by  $\tisW^{(t)}$ in their original specifications.
%Moreover, $\nabla\widehat{\calR}(\tisW^{(t)})$ is defined as:
%\begin{align}
%	\nabla\widehat{\calR}(\tisW^{(t)}):=\frac{\lambda k}{2}\cdot\frac{\langle v_*,\tisW^{(t)} v_*\rangle^{\frac{k}{2}-1}}{\left\|\tisW^{(t)}\right\|_{\text{F}}^{\frac{k}{2}-2}}\cdot v_* v_*^{\top}-\frac{\lambda(k-4)}{2}\cdot\frac{\llangle v_*,\tisW^{(t)} v_*\rrangle^{\frac{k}{2}}}{\left\|\tisW^{(t)}\right\|_{\text{F}}^{\frac{k}{2}}}\cdot\tisW^{(t)}+\tisE^{(t)}.\notag
%\end{align}
%Based on Lemma \ref{lemma:high-prob}, we have that the analysis of control sequence $\{\tisW^{(t)}\}_{t=0}^{T}$ is consistent with that of $\{W ^{(t)}\}_{t=0}^{T}$ with high probability.

%\subsection{Phase I}
%\input{phase_1}

%\subsection{Phase II}
%\input{phase_2_old}

% \subsection{Proof of Main Results in Tensor PCA}
% \input{proof_of_main_convergence_result}

% \subsection{Supplementary}
% \input{Supp}
